Induced superconducting pair correlations in a quasicrystal coupled to a BCS superconductor

In this report, we describe the proximity effect which arises when a quasicrystal is placed in contact with a superconductor. We consider the simplest known model of a quasicrystal, the 1D Fibonacci chain, for which all states are known to be critical. A hybrid ring is made by connecting a finite piece of such a Fibonacci chain to a BCS-type superconductor. Solving the resulting Bogoliubov-de Gennes equations self-consistently, we show that the proximity effect in the Fibonacci chain is long ranged, and that the induced superconducting order carries information on topological properties, namely, the winding numbers of edge states of the Fibonacci chain.

==> iobib2.tex <==
@article{mace2016fractal,
  title={Fractal dimensions of wave functions and local spectral measures on the Fibonacci chain},
  author={Mac{\'e}, Nicolas and Jagannathan, Anuradha and Pi{\'e}chon, Fr{\'e}d{\'e}ric},
  journal={Physical Review B},
  volume={93},
  number={20},
  pages={205153},
  year={2016},
  publisher={APS}
}


@article{baboux2017measuring,
	title={Measuring topological invariants from generalized edge states in polaritonic quasicrystals},
	author={Baboux, Florent and Levy, Eli and Lema{\^\i}tre, Aristide and G{\'o}mez, Carmen and Galopin, Elisabeth and Le Gratiet, Luc and Sagnes, Isabelle and Amo, Alberto and Bloch, Jacqueline and Akkermans, Eric},
	journal={Physical Review B},
	volume={95},
	number={16},
	pages={161114},
	year={2017},
	publisher={APS}
}


@article{aubry1980analyticity,
  title={Analyticity breaking and Anderson localization in incommensurate lattices},
  author={Aubry, Serge and Andr{\'e}, Gilles},
  journal={Ann. Israel Phys. Soc},
  volume={3},
  number={133},
  pages={18},
  year={1980}
}



@article{bellissard1989spectral,
  title={Spectral properties of one dimensional quasicrystals},
  author={Bellissard, J and Iochum, B and Scoppola, E and Testard, D},
  journal={Communications in Mathematical Physics},
  volume={125},
  number={3},
  pages={527--543},
  year={1989},
  publisher={Springer}
}

@article{preprintproximity,
	title={The Proximity Effect in a Superconductor-Quasicrystal Hybrid Ring},
	author={Gautam Rai, Stephan W. Haas and Jagannathan, Anuradha},
	journal={condmat},
	volume={},
	number={Arxiv:1905.08382},
	pages={},
	year={2019},
	publisher={}
}


@article{ledieu2014surfaces,
  title={Surfaces of Al-based complex metallic alloys: atomic structure, thin film growth and reactivity},
  author={Ledieu, Julian and Gaudry, {\'E}milie and Fourn{\'e}e, Vincent},
  journal={Science and Technology of Advanced Materials},
  volume={15},
  number={3},
  pages={034802},
  year={2014},
  publisher={IOP Publishing}
}


